Brownian motion and Symmetrization

In this survey we explore the salient connections made between Brownian motion, symmetrization and complex analysis in the last 60 years starting with Kakutani's paper (1944) equating harmonic measure and exit probability. To exemplify these connections we will survey the techniques used in the literature to prove isoperimetric results for exit probabilities and Riesz capacities.

==> administrative <==
to-do

1)use medicci, the more questions you ask the more paths appear.
2)provide multiple proofs of spitzer's formula: 1)from spitzer's paper 2) from Taylor's pdes 3)from pere's capacities

the goal is to find a proof that will help me understand spitzer's proof.

start by reading
http://www.unc.edu/math/Faculty/met/chap11.pdf


3)use doublespacing or 1.5 spacing

4) why can you take h=t? you showed lim_{t\to \infty}E_{A}(t)-E_{A}(t-h)=\int_{\mathbb{R}^{d}}P_{y}(h\leq \tau_{A^{c}}, \tau_{A}\leq h)dy=h\cdot c. So you already took the limit in t.


5)non-italicized words in theorem environment, how to do it?


6)why \int \int G e(dy) e(x)=e(A)?
lim_{h\to 0}\int\frac{1}{h}P_{y}( \tau_{A}\leq h)

Proved in http://wiki.math.toronto.edu/TorontoMathWiki/index.php/Brownian_Motion_and_Harmonic_functions

Let $l_{x}:=\frac{1}{3}dist(x,\partial A )=\frac{1}{3}\inf\limits_{y\in A}\{|x-y|\}$ and $l_{0}=\inf\limits_{x}l_{x}$, then in \cite[7.7]{Ito_McKean_1965}
\begin{equation*}
P_{x}(\tau_{A}<h)\leq \int_{0}^{h}\frac{1}{(2\pi s^{3})^{\frac{d}{2}}} e^{-\frac{l_{x}^{2}}{2s}}  ds.
\end{equation*}
Therefore, 
\begin{align*}
e_{h}(A^{c})\leq & \frac{1}{h}\int_{A^{c}}P_{y}(\tau_{A}<h)dx\\
\leq &\frac{1}{h}\int_{A^{c}}\int_{0}^{h}\frac{1}{(2\pi s^{3})^{\frac{d}{2}}} e^{-\frac{l_{x}^{2}}{2s}}  ds dx\\
\leq & ~constant \times \frac{1}{h}\int_{0}^{h} \int_{l_{0}}^{\infty}\frac{b^{3}}{(2\pi s^{3})^{\frac{d}{2}}} e^{-\frac{b^{2}}{2s}}  db ds\\
\xrightarrow{h\to 0}&  \int_{l_{0}}^{\infty}\frac{b^{3}}{(2\pi)^{\frac{d}{2}}} \cdot 0~  db ,
\end{align*}
where in the last step we used Lebesgue differentiation theorem.

Find

1) Lectures from Markov Processes to Brownian Motion

Probabilistic Techniques in Analysis
 By Richard F. Bass
